Verifying Text Summaries of Relational Data Sets

We present a novel natural language query interface, the AggChecker, aimed at text summaries of relational data sets. The tool focuses on natural language claims that translate into an SQL query and a claimed query result. Similar in spirit to a spell checker, the AggChecker marks up text passages that seem to be inconsistent with the actual data. At the heart of the system is a probabilistic model that reasons about the input document in a holistic fashion. Based on claim keywords and the document structure, it maps each text claim to a probability distribution over associated query translations. By efficiently executing tens to hundreds of thousands of candidate translations for a typical input document, the system maps text claims to correctness probabilities. This process becomes practical via a specialized processing backend, avoiding redundant work via query merging and result caching. Verification is an interactive process in which users are shown tentative results, enabling them to take corrective actions if necessary. Our system was tested on a set of 53 public articles containing 392 claims. Our test cases include articles from major newspapers, summaries of survey results, and Wikipedia articles. Our tool revealed erroneous claims in roughly a third of test cases. A detailed user study shows that users using our tool are in average six times faster at checking text summaries, compared to generic SQL interfaces. In fully automated verification, our tool achieves significantly higher recall and precision than baselines from the areas of natural language query interfaces and fact-checking.

==> sections/experiments.tex <==
In this section, we present the following experimental results.

\begin{itemize}
	\item \textbf{Section~\ref{sec:sample_articles}. Analysis of Test Cases.} We analyze a total of 34 text documents with 216 claims. The result demonstrates fundamental properties of claims in text documents that substantiate our hypotheses.
	\item \textbf{Section~\ref{sec:unsupervised}. Unsupervised Performance.} Using the test cases, we evaluate a fully automated version of FactChecker with respect to identifying the matching queries. %In 76.3\% of the claims, the FactChecker correctly identifies the SQL query within its top-10 recommendations.
	\item \textbf{Section~\ref{sec:run_time}. Processing Time.} We measure the running times of different versions of FactChecker where we gradually apply the efficient processing strategies. In addition, we evaluate the trade off between the processing overhead versus the accuracy of matching queries.
	\item \textbf{Section~\ref{sec:user_study}. User Study.} The primary goal of FactChecker is to facilitate the process of fact-checking for general users. Thus, the most crucial metric is the performance of FactChecker in real-world situations where users verify claims in text documents. %For example, in our user study, the FactChecker empowered the participants to verify the claims in text documents 5.62$\times$ faster than a standard SQL interface.
\end{itemize}

\subsection{Analysis of Test Cases}
\label{sec:sample_articles}
We analyze 34 publicly available text documents and their associated data sets from various sources including 538, New York Times, Vox, and Stackoverflow. The result reveals fundamental properties of claims in text documents that substantiate our hypotheses. The design of the FactChecker is based on three hypotheses. First, the claims that aggregates over multiple values are prune to errors. Second, the target of newspaper articles are main stream readers, and thus, the matching SQL queries tend to comply with simple templates. Third, a text document usually focuses on a primary topic of interest and only covers few aspects of the data set.

To generate the test cases, we found numerical values from the text documents and annotated them with one of these categories: Correct, Incorrect, Complex, Uncertain, Missing Data, and Not a Claim. We practiced the following procedure for each claim that conform to the SQL template of FactChecker. We formulated the query that matches the context of the claim, executed the query on the data set, and verified its result against the value in the text. If the value matches the query result, we annotated it as \textit{Correct}, and otherwise, as \textit{Incorrect}. As a result, we have a data set of 34 text documents with 216 claims where their correctness and the matching SQL queries are annotated.

\begin{figure*}
	\centering
	\subfigure[Number of correct and incorrect claims in each document. 6.9\% of the claims are incorrect, which are distributed among ten documents out of a total of 34.\label{fig:hypothesis1}]
	{
		\includegraphics[width=0.3\textwidth]{plots/annotationTypeNrAllArticle_Correctness.pdf}
	}
	\subfigure[Distribution of SQL queries according to the number of restrictions. 88.4\% of the matching SQL queries have either zero or one restrictions.\label{fig:hypothesis2}]
	{
		\includegraphics[width=0.3\textwidth]{plots/restrictionRatioStacked.pdf}
	}
	\subfigure[Coverage of claims within a text document with top-N most frequent aggregation function, aggregated column, and restricted column. Note that, more than 84\% of the claims in a document are covered by the top-3 aggregation functions, aggregated columns and restricted columns.\label{fig:hypothesis3}]
	{
		\includegraphics[width=0.36\textwidth]{plots/documentTopNCovergeRatio.pdf}
	}
	\caption{Fundamental properties of claims in text documents that support each of the three hypotheses.\label{fig:analysisTestCases}}
\end{figure*}

%\begin{figure}
%	\includegraphics[width=0.4\textwidth]{plots/annotationTypeNrAllArticle_Correctness.pdf}
%	\caption{Number of correct and incorrect claims in each document.\label{fig:annotation_dist}}
%\end{figure}

%\begin{figure}
%	\includegraphics[width=0.35\textwidth]{plots/restrictionRatioStacked.pdf}
%	\caption{Distribution of SQL queries according to the number of restrictions. 88.4\% of the matching SQL queries have either zero or one restrictions.\label{fig:dist_restriction}}
%\end{figure}

%\begin{figure}
%	\includegraphics[width=0.45\textwidth]{plots/documentTopNCovergeRatio.pdf}
%	\caption{Coverage of claims within a text document with top-N most frequent aggregation function, aggregated column, and restricted column. Note that, on average, more than 80\% of the claims in an article use one of the top-2 aggregation functions. Likewise, more than 84\% of the claims are covered by one of the top-3 aggregated columns and restricted columns.\label{fig:topNCoverge}}
%\end{figure} 

\textbf{Hypothesis 1.} First, Figure~\ref{fig:hypothesis1} shows the number of correct and incorrect claims in each article. Note that these claims are associated with matching queries that comply to the SQL template of FactChecker. Surprisingly, despite the notion that the claims in newspaper articles or summaries of surveys will be accurate, 6.9\% of all claims are actually erroneous. Moreover, among 34 text documents, ten of them have at least one incorrect claim. This finding supports our first hypothesis that the aggregations over multiple values are prune to errors. We have contacted the authors of text documents by email to verify whether the incorrect claims are truly erroneous. Although not all authors have replied, we received several emails indicating that these claims are actually errors. More importantly, all incorrect claims that we verified with the authors conformed to our initial annotations. Some of the typical errors include rounding errors, counting errors, and unsynchronized data set.

\textbf{Hypothesis 2.} Next, Figure~\ref{fig:hypothesis2} depicts the distribution of the matching SQL queries according to the number of restrictions. 88.4\% of the SQL queries are simply structured queries with zero or one restrictions. Note that, the data set contains only four claims from Vox, and thus, it cannot be seen as a typical case.

\textbf{Hypothesis 3.} In Figure~\ref{fig:hypothesis3}, the top-N most frequent aggregation functions, aggregated columns, and restrictions of matching SQL queries apply to most of the claims in a document. The coverage over the claims grows rapidly in the first top-3 in all cases which becomes more than 84\%. This result demonstrate that an article mostly focuses on a small area of interest (e.g., using small number of aggregation functions, aggregated columns, and restricted columns) among the vast amount of SQL queries that are applicable to the data set.


\subsection{Unsupervised Performance}
\label{sec:unsupervised}

\begin{figure*}
	\centering
	\subfigure[Correctness of claims.\label{fig:topNQueries_Correctness}]
	{
		\includegraphics[width=0.3\textwidth]{plots/topNQueriesRatio_Correctness.pdf}
	}
	\subfigure[Different aggregation functions.\label{fig:topNQueries_Function}]
	{
		\includegraphics[width=0.3\textwidth]{plots/topNQueriesRatio_Function.pdf}
	}
	\subfigure[Number of restrictions.\label{fig:topNQueries_Restriction}]
	{
		\includegraphics[width=0.3\textwidth]{plots/topNQueriesRatio_Restriction.pdf}
	}
	\caption{Accuracy of top-N mostly likely query recommendations.\label{fig:topNQueries}}
\end{figure*}

\begin{figure}
	\includegraphics[width=0.3\textwidth]{plots/nrPossibleQueries.pdf}
	\caption{Total number of SQL query candidates that comply with the SQL query template used in FactChecker.\label{fig:possibleQueries}}
\end{figure}

\textbf{Overall Accuracy.}
We present rigorous experimental results on a set of 34 text documents with respect to the accuracy of FactChecker in identifying the underlying SQL query that matches the claim. Figure~\ref{fig:topNQueries} presents the accuracy in terms of the top-N mostly likely SQL query recommendations. To be specific, the accuracy denotes whether the SQL query that matches the context of the claim appears in the first N query recommendations with the highest probabilities. Red line indicates the overall accuracy on the total of 216 claims. It is shown that the top-1 SQL query achieves 54.74\% coverage among all statistics, an impressive number which even reaches 71.55\% and 76.29\%, respectively, in the top-5 and top-10 query recommendations. This is a significant performance when compared against the total number of SQL query candidates that could be generated for each data set. Figure~\ref{fig:possibleQueries} illustrates the number of SQL query candidates, in log scale, that comply with the SQL template used in FactChecker. For instance, the article with the largest dataset have $1.08\times10^{12}$ SQL query candidates where top-10 query recommendations only accounts for $9.3\times10^{10}$\% of the possible cases.

\textbf{Accuracy by Different Categories.}
In Figure~\ref{fig:topNQueries}, we categorized the claims according to 1) their correctness, 2) the aggregation function of the matching query, and 3) the number of restrictions. Figure~\ref{fig:topNQueries_Correctness} shows that the FactChecker benefits from those claims that are actually correct demonstrating a high accuracy of 80.6\% in top-10 recommendations. In contract, the system suffers a lower accuracy of 18.8\% on incorrect claims, which is a natural consequence of the FactChecker exploiting the particularity of fact checking that most claims in text documents are actually correct. As shown in Figure~\ref{fig:topNQueries_Function}, the FactChecker performs relatively well on SUM and PERCENTAGE aggregates while the difference among aggregation functions is small compared to other categories. In Figure~\ref{fig:topNQueries_Restriction}, the claims with zero or one restrictions exhibit high accuracies. On the other hand, the FactChecker performs less well on the SQL queries with two restrictions because the system needs to correctly identify an increased number of query fragments.

\begin{figure}
	\includegraphics[width=0.35\textwidth]{plots/accuracyPerLucene.pdf}
	\caption{Accuracy of FactChecker with varying hierarchies of keyword context.\label{fig:accuracyPerLucene}}
\end{figure}

\textbf{Accuracy by Hierarchies of Lucene Input.}
Figure~\ref{fig:accuracyPerLucene} illustrates the accuracy of different versions of FactChecker with respect to the keyword context. We gradually added each layer of keyword context to measure the affect of the top-1, top-5, and top-10 mostly likely SQL queries. It could be easily seen that, for top-1 query, the accuracy increases accordingly as we include more layers of keyword context. For top-5 and top-10, there are two significant improvements when we add the previous sentence and the headlines to the keyword context hierarchy. In all cases, our assumption that the hint about the relevant database elements are given in different levels of the document hierarchy is justified.



\subsection{Processing Time}
\label{sec:run_time}

\begin{figure} % Need to add 'x 23' with arrows in the plots
	\includegraphics[width=0.3\textwidth]{plots/performanceAllArticles.pdf}
	\caption{Performance improvement by applying different strategies for SQL query execution (in log scale).\label{fig:performanceAll}}
\end{figure}

\begin{figure}
	\includegraphics[width=0.3\textwidth]{plots/timePerComponentBySize.pdf}
	\caption{Ratio of processing time per component of FactChecker. The time shown above each bar indicates the average processing time for each category. For large data sets, the SQL query execution time dominates the FactChecker processing time.\label{fig:timePerComponent}}
\end{figure}

\textbf{Efficient Processing Strategies.}
We present the processing time of different versions of FactChecker with varying processing strategies. \textit{Naive} version separately executes each individual query candidate which aggregates into one value, instead of combining them to one cube query. \textit{Merging} version merges SQL queries into cube queries but does not utilize caching. On the other hand, \textit{caching} version takes into account the similarity between the cube queries issued across different claims and also different EM iterations. Last, \textit{incremental} version incrementally increases the dimension of cube query starting from the mostly likely restricted column in order to exploit early stopping. Note that each version generates exactly the same number of aggregated values from the database. As shown in Figure~\ref{fig:performanceAll}, we observe speed ups of 114$\times$ and 2.08$\times$ between two consecutive versions respectively, in terms of query execution time. We use the fastest \text{caching} version of FactChecker to measure the processing time for other experiments. Figure~\ref{fig:timePerComponent} shows that query execution time dominates the processing time when it comes to large data sets whose sizes are above 10MB.

\begin{figure*}
	\centering
	\subfigure[Number of aggregation functions (1 \textasciitilde{} 5).\label{fig:timeAccuracy_AggFunc}]
	{
		\includegraphics[width=0.235\textwidth]{plots/timeAccuracy_AggFunction.pdf}
	} 
	\subfigure[Number of aggregated columns (1 \textasciitilde{} 20).\label{fig:timeAccuracy_AggColumn}]
	{
		\includegraphics[width=0.235\textwidth]{plots/timeAccuracy_AggColumn.pdf}
	}
	\subfigure[Number of restricted columns (1 \textasciitilde{} 10).\label{fig:timeAccuracy_RestrictColumn}]
	{
		\includegraphics[width=0.235\textwidth]{plots/timeAccuracy_RestrictColumn.pdf}
	}
	\subfigure[Number of EM iterations (1 \textasciitilde{} 10).\label{fig:timeAccuracy_MaxIterationEM}]
	{
		\includegraphics[width=0.235\textwidth]{plots/timeAccuracy_MaxIterationEM.pdf}
	}
	\caption{Accuracy of FactChecker with varying amount of processing overhead. As the FactChecker utilize more processing power, also the accuracy generally increases except for the number of restricted columns.\label{fig:timeAccuracy}}
\end{figure*}

\textbf{Trade Off between Processing Overhead and Accuracy.}
Figure~\ref{fig:timeAccuracy} depicts the trade off between processing overhead and accuracy. This trade off is a unique property that only applies to the fact-checking task in contract to the typical natural language querying. We are given not only a natural language representation of the matching query, but also a plausible result of that query. Therefore, we can overcome the challenges in natural language understanding by trying out a large amount of query candidates.

\subsection{User Study}
\label{sec:user_study}
The core purpose of FactChecker is to increase user performance when fact-checking text documents. Therefore, the most important question to ask is how well does the FactChecker support users in verifying claims under real-world circumstances. More precisely, we measure the speed up achieved by utilizing out tool compared to a standard SQL interface.

We conducted a user study to evaluate the performance of FactChecker in real-world situations. The participants of the study were asked to verify the claims in real articles from various sources, including 538, New York Times, and Stackoverflow, while using either of the two tools: the FactChecker or an SQL interface. The goal of the study was to 1) measure how fast the users perform with our tool compared to an SQL interface, 2) observe in what way the users benefit from using FactChecker, and 3) receive qualitative feedbacks about FactChecker.

\textbf{Participants.}
We recruited eight participants where seven of them are students majoring Computer Science and one studies other discipline. According to the survey filled out by each participant, one has no experience in SQL, four are beginners, two are intermediate, and one has an advanced knowledge.

\textbf{Data set.}
The data set consists of six real-world text documents from three sources. Three articles are from 538, one is from New York Times, and two are survey summaries from Stackoverflow. There are two long articles and four short articles where long articles have at least 15 claims while short articles have 5\textasciitilde{}10 claims. We separated the articles into two sets where each set contains one long article and two short articles. Each user completes both sets but using different tools.

\textbf{Process.}
First, we give a five-minute introductory tutorial of the FactChecker. The actual presentation time which we measured during the user study was exactly 5 minutes and 33 seconds. Then, we divide the participants into two groups. One group starts with the FactChecker while the other group starts with an SQL interface. Moreover, the participants switch tools after the completion of each article. These protocols prevent the participants' familiarization with the task from affecting the performances of using different tools. 
Next, each user starts verifying the claims in an article under a time limit, 20 minutes for a long article and 5 minutes for a short article. After the time runs out, the system automatically stops and the users proceed to the next article until they finish all six articles. Last, each participant fills out a survey with rating-scaled and open-ended questions.

\textbf{Metrics.}
During the user study, we have provided an interface with the functionality to mark each claim as either correct or incorrect. The system logs the time when a participant marks up a claim. We use these time stamps to determine how fast the user verified the claims.
Nevertheless, we have to make sure that each verification of a claim is based on the result of executing the matching query rather than a mere guess. For this purpose, we also logged every SQL queries the participants have executed. Only when the user have executed the matching query was the verification of a claim confirmed.

\begin{figure*}
	\centering
	\subfigure[Stackoverflow 2016.\label{fig:userStudy_StackOverflow2016}]
	{
		\includegraphics[width=0.3\textwidth]{plots/userStudy_StackOverflow2016.pdf}
	}
	\subfigure[flying etiquette survey.\label{fig:userStudy_flyingetiquettesurvey}]
	{
		\includegraphics[width=0.3\textwidth]{plots/userStudy_flyingetiquettesurvey.pdf}
	}
	\subfigure[Stackoverflow 2015.\label{fig:userStudy_StackOverflow2015}]
	{
		\includegraphics[width=0.3\textwidth]{plots/userStudy_StackOverflow2015.pdf}
	}
	\subfigure[elo blatter. \label{fig:userStudy_eloblatter}]
	{
		\includegraphics[width=0.3\textwidth]{plots/userStudy_eloblatter.pdf}
	} 
	\subfigure[Sunday Shows.\label{fig:userStudy_SundayShowsd}]
	{
		\includegraphics[width=0.3\textwidth]{plots/userStudy_SundayShows.pdf}
	}
	\subfigure[hiphop candidate lyrics.\label{fig:userStudy_hiphopcandidatelyrics}]
	{
		\includegraphics[width=0.3\textwidth]{plots/userStudy_hiphopcandidatelyrics.pdf}
	}
	\caption{Number of correctly verified claims as time proceeds. Bold line indicates the average over the participants using the same tool. In all test cases, participants correctly verifies the claims in a much faster rate using the FactChecker compared to an SQL interface.\label{fig:userStudyPerArticle}}
\end{figure*}

\begin{figure*} % Need to add 'x 23' with arrows in the plots
	\centering
	\subfigure[Users.\label{fig:userStudyPerMinute_User}]
	{
		\includegraphics[width=0.3\textwidth]{plots/userStudyPerMinuteByUser.pdf}
	}
	\subfigure[User SQL expertise.\label{fig:userStudyPerMinute_SQLExperience}]
	{
		\includegraphics[width=0.3\textwidth]{plots/userStudyPerMinuteBySQLExperience.pdf}
	}
	\subfigure[Articles.\label{fig:userStudyPerMinute_Article}]
	{
		\includegraphics[width=0.3\textwidth]{plots/userStudyPerMinuteByArticle.pdf}
	}
	\caption{Number of correctly verified claims per minute. In all cases, the FactChecker performs better than an SQL interface, on average 5.62$\times$ faster in verifying the claims. \label{fig:userStudyPerMinute}}
\end{figure*}

\textbf{Evaluation (Performance).}
Figure~\ref{fig:userStudyPerArticle} depicts the number of correctly verified claims as time proceeds. In all article, it is clearly shown that the participants using the FactChecker were able to verify more claims than those using a SQL interface. The speed up of FactChecker becomes more evident in Figure~\ref{fig:userStudyPerMinute}. Figure~\ref{fig:userStudyPerMinute_User} compares the number of correctly verified claims per minute between different tools. Note that every user performs better when using FactChecker with an average 5.62$\times$ speed up. We grouped this result with respect to the different SQL expertises of users in Figure~\ref{fig:userStudyPerMinute_SQLExperience}. With one exception (Advanced, FactChecker), the number of correctly verified claims increases as the expertise deepens regardless of the tool, where the FactChecker enjoys a steeper incline. Even for each article, the FactChecker users are always superior with an average speed up of 3.79$\times$, as shown in Figure~\ref{fig:userStudyPerMinute_Article}.

\begin{figure}
	\includegraphics[width=0.4\textwidth]{plots/userStudyRatingComparison_SQLExperience.pdf}
	\caption{User rating of the FactChecker compared to an SQL interface.\label{fig:userStudyUsabilityRating}}
\end{figure}

\textbf{Evaluation (Usability).}
Figure~\ref{fig:userStudyUsabilityRating} presents the summary of the usability rating question in the survey. It shows a high average rating of 4.75 on the question asking for the overall usability of the FactChecker compared to a SQL interface. The rating 5 denotes ``much better'' while the rating 1 indicates ``much worse.'' Note that the system has a very high average rating of 4.875 in verifying correct claims whereas a relatively low, but still high, rating of 4.375 in verifying incorrect claims.

In response to the open-ended questions in the survey, the participants gave positive answers. For example, one participant commented: ``\textit{Shortened time considerably. Very Very friendly to non-cs majors. Interface is very simple and easy to follow. I was able to finish all the ones that I used Face Checker before the time ran out so it's awesome. If I had to choose between SQL and Face Checker, I'd choose Fact Checker any day.}`` Some other responses include: ``\textit{Really liked that it showed the result of the recommended queries. The suggestions made it very easy to create custom queries,}'' ``\textit{It was very quick and easy to verify correct statistics when it formulated the correct query,}'' and ``\textit{It select the correct query in most time. Good.}''

==> sections/interface.tex <==

\begin{figure*}
\centering
% Let's scale down screenshots enough to fit all subfigures into one row
\subfigure[Entry screen: text input and data set selection.\label{entryFig}]
{\includegraphics[width=0.19\textwidth]{figures/screenshot1.png}} % No Cornell logo!!
\subfigure[Marked up claims after initial processing.\label{markupFig}]
{\includegraphics[width=0.19\textwidth]{figures/screenshot2.png}}
\subfigure[Display of query description upon hovering.\label{queryFig}]
{\includegraphics[width=0.19\textwidth]{figures/screenshot3_cursor.png}}
\subfigure[Select query from top-5 likely candidates.\label{topFig}]
{\includegraphics[width=0.19\textwidth]{figures/screenshot4.png}}
\subfigure[Construct query by selecting from fragments.\label{fragmentsFig}]
{\includegraphics[width=0.19\textwidth]{figures/screenshot5.png}}
\caption{Screenshots from the FactChecker user interface.\label{interfaceFig}}
\end{figure*}

%We describe how users interact with the FactChecker. A user might for instance be a data journalist who uses the FactChecker to verify claims in his or her article before submission. 

%Optionally, a relational database might come with a data dictionary that associates database elements (e.g., columns or values) with short textual descriptions. The FactChecker offers a parser to automatically extract information from popular data dictionary formats (e.g., used for the US Census data sets). If no data dictionary is specified, only the names of database elements are used for interpreting natural language claims.

Users must first load the relational database to which a text refers to. After loading the data, users enter a natural language text that contains claims on the data (see Figure~\ref{entryFig}). The input might contain HTML markup to structure the document into sections and subsections. If present, such markup can be exploited to increase checking accuracy (see Section~\ref{matchingSec}). After entering a text, users select the data set against which the text should be fact-checked. Before the actual checking stage, users may correct the automated claim identification heuristic by selecting or de-selecting check-worthy text passages. 

%They can choose from one of the previously loaded data sets. After selection, users click on the ``Verify'' button to start the fact-checking process.

%This could for instance be a newspaper article in case of a data journalist user. In addition to raw text, 

As explained in more detail later, the system now learns the document focus, evaluates queries, and determines likely query candidates for each claim. This typically takes a couple of seconds, a few tens of seconds for large data sets. Afterwards, the user is presented with a marked up version of the input text (see Figure~\ref{markupFig}). Claims have been identified and tentatively marked as correct (indicated by light green markup) or incorrect (indicated by light red markup). Of course, this classification is dependent upon the system finding the right SQL query for a natural language claim.

%If that interpretation matches the claim, the user may simply leave it as it is or click on the check mark in the left upper corner. That marks the claim as user-verified and the markup turns into a solid green (or solid red). 

Upon hovering over a marked up claim, users are presented with a natural language description of the SQL query that the system associates with the claim (see Figure~\ref{queryFig}). While the system detects the right query in the majority of cases (see Section~\ref{experimentsSec}), the recognized query may not match the claim in other cases. Then, the system supports users in taking corrective actions. 

Even if the most likely query identified by the system for a given claim does not match the actual query, the right query is typically contained within the top-5 likely query candidates. Users can access the top-5 or top-10 most likely query candidates calculated by the system (see Figure~\ref{topFig}). As a last resort, users may construct the right query by combining query fragments. The system proposes likely fragments to facilitate that process (see Figure~\ref{fragmentsFig}). 

%for each claim click on the button ``View More Queries'' to obtain a list of the five most likely query candidates, together with the results of evaluating those queries on the database (see Figure~\ref{topFig}). If a user selects one of those queries, the claim is automatically marked up as (user-verified) correct or incorrect based on the query result. If the right query is not within the top-5, users may view the top-10 queries by clicking on the ``View Even More Queries'' button. Alternatively, users may construct the right query, using likely query fragments proposed by the system.

%To initiate that process, users click on the ``Build Query'' button. They can in the following select an aggregation function, the system ranks the proposed functions by their likelihood based on text analysis. Then, users select the column over which we aggregate (see Figure~\ref{fragmentsFig}). Again, the system ranks columns by their likelihood and colors them based on their probability. Finally, users have the possibility to select restrictions (i.e., equality predicates on columns), ranked again by their likelihood. Finally, the system evaluates the user-defined query and marks up the claim in the text document, based on whether or not the query result matches the one claimed in text.

The end result of fact checking is a categorization of claims into correct and incorrect ones. In addition, claims have been mapped to queries and the system has determined evaluation results for them. They can be used to correct erroneous claims. After users have finished a fact-checking session, they can store the result in order to continue later or to revise the text based on it.

==> sections/intro.tex <==

%A wealth of information is nowadays available in the form of relational data sets. However, the largest part of the population never accesses raw data. 

A majority of the population never accesses raw relational data. Instead, most people rely on textual summaries that contain aggregate information on such data sets. Examples range from New York Times articles summarizing trends in the newest US Census data set to company-internal executive reports summarizing quarterly sales. In all those cases, the same question arises: how can we trust a textual summary to accurately reflect the underlying data? In this paper, we present a ``FactChecker'' for text summarizing relational data, which partially answers this question. \blue{A link to our online demo featuring all test cases used for this paper will be available in a camera-ready version of our paper.}
% A demo featuring all test cases used for this paper can be found online~\cite{CornellDemo, CornellHP}.

Prior work~\cite{HassanZ17} has focused on verifying claims that have already been verified or refuted by human fact checkers. Our goal is to fact-check based on raw relational data instead. We verify claims about numerical aggregates for which no ground truth is readily available. Instead, verifying a claim requires evaluating SQL queries that the claim implicitly describes. Our system is similar in spirit to a spell checker: where a spell checker supports authors in avoiding typos and grammatical mistakes, the FactChecker helps authors to avoid inaccurate factual claims. 

%Our focus is not necessarily on adversarial fact-checking (i.e., verifying if claims made by a third person are accurate). We primarily want to support authors of textual summaries in avoiding unnecessary factual mistakes.

%We verify natural language claims stating that the result We verify claims on numerical aggregates for which ground truth is not explicitly stored

The FactChecker is semi-automated in a similar sense as a spell checker is semi-automated. A spell checker marks up potential typos, thereby focusing the author's attention on a small part of the document to significantly reduce verification overheads. Still, authors need to verify whether marked up words represent actual typos or for instance unusual names of persons that are not in the dictionary. The FactChecker works in a similar manner: starting from a text document and an associated database, it automatically spots check-worthy claims about the data, identifies SQL queries matching the claim intent, executes those queries and finally marks up text passages where query results seem to contradict the text. Users are presented with natural language descriptions of the SQL queries that the system maps claims to. While the system automatically maps claims to the right queries in the majority of cases, users can correct the system's interpretation otherwise. In the latter case, the FactChecker still proposes runner up queries in decreasing order of likelihood, or supports users in selecting the right query themselves by proposing likely query fragments.

The problem of fact-checking might seem close to the problem of natural language querying (which has recently received significant attention in the database community~\cite{Agrawal2002, Li2014, Saha2016}). In both case, the goal is to map natural language expressions to SQL queries. There are however several fundamental differences between the problem of natural language query translation and the problem of fact-checking. First, in fact-checking, we are not only given a natural language query but also a claimed result of that query. Second, instead of a single query, we are given an entire text document containing multiple, related claims. 

Our system design is intrinsically based on both particularities. Since we are given claimed results together with queries (in natural language representation), we can partially trade challenges in natural language understanding for processing overheads. More precisely, if we can only narrow down the set of query candidates behind a natural language claim, we can evaluate them and compare their results to the claimed one. At least in case of accurate claims, a matching result provides strong evidence for one specific interpretation of the natural language claim. As query candidates for the same claim tend to be similar, we can furthermore apply techniques such as query merging or caching to increase processing efficiency and finally our accuracy.

This does of course not help us in case of erroneous claims. However, for those we can exploit the fact that we are given an entire text document instead of a single claim. Our initial intuition was that text documents tend to focus on a limited number of aspects of a given data set (e.g., one specific New York Times article about the US Census data set could focus on income inequalities while ignoring other parts of the data). We have verified that intuition later by analyzing a multitude of real reports and articles (more details are provided in Section~\ref{testCasesSub}). We therefore link natural language claims in a document by a probabilistic model, based on the assumption that claims in the same document tend to have similarities. This gives us the possibility to exploit what we learn about one claim to bias our belief about another. 

More precisely, the FactChecker takes as input one relational database and one text document, containing factual claims about the database (among other text). We currently focus on fact-checking claims that can be expressed as SQL queries with aggregates and conjunctive equality predicates. Our initial hypothesis was that this type of claim is at the same time common as well as error-prone (since precise numbers are harder to remember than relative tendencies and since aggregates cannot be verified without actually executing queries on the data). We confirmed this hypothesis by a detailed analysis of various newspaper articles and other reports (more details are given in Section~\ref{testCasesSub}). 

%We also perform various string manipulations to extract keywords from abbreviated or concatenated identifiers in the data set (e.g., treating common cases where column names consist of a combination of keywords that are not separated by dedicated delimiters). 

In a first step, the FactChecker indexes query fragments formed from database elements (e.g., we form equality predicates from literals in the database). We exploit data sets such as WordNet in order to associate database entries with synonyms and related keywords. As a result, we obtain for each query fragment a set of keywords. We store each of those keyword sets as a small document that is indexed via an information retrieval engine. %(we use Apache Lucene in our current implementation). 

%We use dependency-parsing in order to identify the keywords within a claim sentence that are most relevant for a specific claim (the same sentence may in fact contain multiple claims, and keywords in the same sentence might have different relevance for different claims). 

In the second step, the FactChecker analyzes the input text document. We use a simple method to identify potential claims about numerical aggregates of the data. For each claim, we analyze the surrounding text in order to identify the most relevant keywords. We weight keywords in the same sentence based on the dependency parse tree. Also, we exploit the structure of the input text to identify more, potentially relevant keywords. For instance, if the document is structured into sections and subsections then keywords in the headlines of all containing (sub-)sections are interesting. Based on the weighted set of keywords associated with one specific claim, we query the information retrieval engine to rank query fragments.

Claim-specific relevance scores for each query fragment form the input to a probabilistic model. This model is based on the assumption that claims in the text document have a certain focus. More precisely, we assume that the queries underlying different claims in the same document have all been drawn from the same probability distribution. Of course, we initially do not know the query distribution underlying the document. Also, we do not initially know the queries behind the claims in the document (from which the document query distribution could be easily inferred). We use an expectation-maximization approach to learn the document distribution as well as the most likely query for each claim. Starting from a uniform distribution, we iteratively infer most likely SQL queries for each claim from the document distribution, and infer the document distribution from the most likely claim queries. 

Keywords alone are insufficient to reliably interpret the document text. Our key insight is that fact-checking allows to reduce uncertainty in natural language analysis by executing likely query candidates. We therefore interleave model learning and query evaluations. If a query candidate evaluates to a result claimed in the text (or to a result that might be rounded to the claimed result), we treat that fact as an important signal for model learning. The more queries we can evaluate under run time constraints, the more accurate our query interpretations will be. We exploit the fact that candidate queries for the same claim (or even for different claims within the same document) are typically similar. We merge different queries for the same claim or even for different claims into single SQL queries, thereby reducing redundant work by orders of magnitude. %We use caching to share work over different iterations of the expectation-maximization algorithm. %Also, we use an incremental evaluation approach that stops evaluations early if it becomes clear that result values would not match the value claimed in the text.

We obtain a probability distribution over queries for each claim in the document. Based on the most likely query for each claim, we tentatively mark up each claim as either correct or incorrect. The results are presented to users by marking up verified or potentially erroneous text passages. Users can verify the FactChecker's interpretations, correct them if necessary, and obtain guidance on alternative query candidates or likely query fragments. 

We tested the FactChecker on a set of 53 text documents that summarize relational data sets. Our test cases include for instance newspaper articles by 538 and the New York Times, as well as summaries of developer surveys by Stack Overflow. We did not alter the articles nor did we apply any pre-processing on the associated data. Using the FactChecker, we were able to identify erroneous claims in 17 articles. The most likely SQL query identified by FactChecker for each claim is the right one in more than half of the cases. In more than 68\% of the cases, the right query is one of the top ten queries shown to users. This accuracy becomes only possible due to efficient processing strategies that allow us to evaluate hundred thousands of similar query candidates per document, even on large data sets. We show in our experiments that our processing strategies improve query throughput by multiple orders of magnitude.

%This is particularly impressive, given that we experimented with first time users who were only given a six minute introduction to FactChecker. 

We executed a user study showing that a user verifies text documents in average about six times faster when using the FactChecker than when using generic SQL interfaces. Also, in fully automated mode, we obtain significantly better recall and precision than state-of-the-art baselines from the areas of natural language query interfaces and fact-checking. We summarize our original scientific contributions:
\begin{itemize}
\item We introduce the problem of checking aggregates in natural language summaries of relational data.
\item We describe a novel system to perform relational fact-checking based on a combination of natural language analysis, learning, and smart ``brute-force'' query evaluations of likely candidates.
\item We report experimental results on many real text documents summarizing relational data sets. We compare against generic query interfaces as well as baselines from the areas of natural language query interfaces and fact-checking. %The experiments cover precision of purely automated fact-checking, processing overheads, and the results of a detailed user study. %showing that novice users can benefit significantly from our tool.
\end{itemize}

The reminder of this paper is organized as follows. We formalize our problem model in Section~\ref{problemSec}. In Section~\ref{overviewSec}, we give an overview of the FactChecker system. In Section~\ref{matchingSec}, we describe how we use keywords to map textual claims to potentially relevant query fragments. We describe our probabilistic model, inferring probability distributions over queries, in Section~\ref{modelSec}. In Section~\ref{querySec}, we describe how we efficiently evaluate similar query candidates to verify claims on the database. Section~\ref{experimentsSec} presents detailed experimental results on real articles and associated data. Finally, we describe related work in Section~\ref{relatedSec}. %and conclude in Section~\ref{conclusionSec}.

%We describe the user interface in Section~\ref{interfaceSec}. 

%Finally, while recent research on natural language query interfaces aims at supporting complex queries (e.g., queries that use nesting), the queries underlying claims in text summaries tend to be relatively simple, in order to be understood by mainstream readers.

%This means that we can partially trade natural language understanding challenges for processing overheads, at least for accurate claims: if we can narrow down the set of query candidates to a reasonable number, we can execute them and compare their results to the one in the claim. Second, 

\begin{comment}
(Problem Definition) Given textual summaries of relational data sets, how can we verify the statistical claims within the text whether they truly match the underlying data?
 
(Why Important) Statistical claims that summarize relevant data sets are ubiquitous in various documents including executive summaries, census publications, technique reports, and newspaper articles. In particular, the concept of data journalism has emerged recently, which led to the establishment of data journalism brands in three major news organizations.
 
(Previous Problem) Nevertheless, despite the growing prominence of data-driven documents, there has been little effort to verify the textual summaries against their associated data sets, mostly due to the onerous effort required in double-checking the statistical claims. Lack of such verification leaves the documents prone to human errors and degrade their credibility.
 
(Our Method) In this context, we present a novel tool FactChecker, similar in spirit to a spell checker, to ``fact-check'' textual summaries of relational data sets. 
Such tools could be used, for instance, by data journalists in order to increase productivity and decrease factual error rates. To the best of our knowledge, this is the first semi-automatic fact-checking tool that directly utilizes the relational data stored in database to verify the statistical claims in natural language text.
By 1) extracting keywords from the document, 2) formulating relevant SQL query candidates, and 3) learning the document-specific probability distribution over the queries, the system identifies the most likely SQL queries, for each claim, that reproduce the statistical value referred by the document.
 
(Impressive Experimental Results) In our user study, the participants using our system verify the statistical claims 5.6$\times$ faster compared to those using an SQL interface. Moreover, when distinguishing wrong claims, FactChecker users demonstrate a 100\% recall with 91\% precision while SQL interface users show a low 29\% recall with 46\% precision. In an experimental evaluation over 40 documents, a total of 241 statistical claims, FactChecker finds the SQL query that matches the text 1) within its top-1 most likely query in 52.7\% of the claims, and 2) within its top-10 queries in 74.3\% of the claims.
\end{comment}

==> sections/tikzPlots.tex <==

\begin{comment}
\begin{figure}
\begin{tikzpicture}[mark size=0.5pt]
\begin{groupplot}[width=3.9cm, height=3.5cm, %
group style={group size = 3 by 1, y descriptions at=edge left, horizontal sep=0.1cm}, %
ymin=0, ymax=100, xlabel={Top-N Queries}, ylabel={Accuracy}, ylabel near ticks, ymajorgrids,%
legend style={font=\small, at={(0.5,1.05)}, anchor=south}]
\nextgroupplot[legend entries={Total, Correct, Wrong}]
\addplot table[x index=0, y index=1, col sep=comma] {plots/topNQueriesRatio_Correctness.txt};
\addplot table[x index=0, y index=2, col sep=comma] {plots/topNQueriesRatio_Correctness.txt};
\addplot table[x index=0, y index=3, col sep=comma] {plots/topNQueriesRatio_Correctness.txt};
\nextgroupplot[legend entries={Total, \%, Count, C.D., Sum, Avg.}, legend columns=2]
\addplot table[x index=0, y index=1] {plots/topNQueriesRatio_FunctionPGF.txt};
\addplot table[x index=0, y index=2] {plots/topNQueriesRatio_FunctionPGF.txt};
\addplot table[x index=0, y index=3] {plots/topNQueriesRatio_FunctionPGF.txt};
\addplot table[x index=0, y index=4] {plots/topNQueriesRatio_FunctionPGF.txt};
\addplot table[x index=0, y index=5] {plots/topNQueriesRatio_FunctionPGF.txt};
\addplot table[x index=0, y index=6] {plots/topNQueriesRatio_FunctionPGF.txt};
\nextgroupplot[legend entries={Total, 0-Preds, 1-Pred, 2-Preds}]
\addplot table[x index=0, y index=1, col sep=comma] {plots/topNQueriesRatio_Restriction.txt};
\addplot table[x index=0, y index=2, col sep=comma] {plots/topNQueriesRatio_Restriction.txt};
\addplot table[x index=0, y index=3, col sep=comma] {plots/topNQueriesRatio_Restriction.txt};
\addplot table[x index=0, y index=4, col sep=comma] {plots/topNQueriesRatio_Restriction.txt};
\end{groupplot}
\end{tikzpicture}
\caption{test}
\end{figure}
\end{comment}

\begin{comment}
\begin{figure}
\begin{tikzpicture}[mark size=1pt]
\begin{groupplot}[width=3.75cm, height=3.5cm, %
group style={group size = 3 by 2, x descriptions at=edge bottom, ylabels at=edge left, horizontal sep=0.3cm}, %
ymin=0, xlabel={Time (s)}, ylabel={\#Claims Verified}, ylabel near ticks, ymajorgrids, xmajorgrids, legend to name=userVerifiedLegend]
\nextgroupplot[title={Stack Overflow 16}]
\addplot table[x index=0, y index=7, col sep=comma] {plots/userStudy_StackOverflow2016.txt};
\addplot table[x index=0, y index=8, col sep=comma] {plots/userStudy_StackOverflow2016.txt};

\nextgroupplot[title={Stack Overflow 15}]
\addplot table[x index=0, y index=9, col sep=comma] {plots/userStudy_StackOverflow2015.txt};
\addplot table[x index=0, y index=10, col sep=comma] {plots/userStudy_StackOverflow2015.txt};

\nextgroupplot[title={Elo Blatter}]
\addplot table[x index=0, y index=9, col sep=comma] {plots/userStudy_eloblatter.txt};
\addplot table[x index=0, y index=10, col sep=comma] {plots/userStudy_eloblatter.txt};

\nextgroupplot[title={Flying Etiquette}]
\addplot table[x index=0, y index=7, col sep=comma] {plots/userStudy_flyingetiquettesurvey.txt};
\addplot table[x index=0, y index=8, col sep=comma] {plots/userStudy_flyingetiquettesurvey.txt};

\nextgroupplot[title={Sunday Shows}]
\addplot table[x index=0, y index=8, col sep=comma] {plots/userStudy_SundayShows.txt};
\addplot table[x index=0, y index=9, col sep=comma] {plots/userStudy_SundayShows.txt};

\nextgroupplot[title={Hiphop Candidates}, legend entries={FactChecker (Avg), SQL (Avg)}, legend columns=2]
\addplot table[x index=0, y index=9, col sep=comma] {plots/userStudy_hiphopcandidatelyrics.txt};
\addplot table[x index=0, y index=10, col sep=comma] {plots/userStudy_hiphopcandidatelyrics.txt};
\end{groupplot}
\end{tikzpicture}

\ref{userVerifiedLegend}
\caption{a}
\end{figure}


\begin{figure}
\begin{tikzpicture}[mark size=1pt]
\begin{groupplot}[width=4.5cm, height=3.5cm, %
group style={group size = 2 by 1, x descriptions at=edge bottom, ylabels at=edge left, horizontal sep=0.4cm}, %
ymin=0, ylabel={\#Verified/Minute}, ylabel near ticks, ymajorgrids, legend to name=userThroughputLegend, ybar=0pt, xtick=data, x label style={at={(0.5,-0.25)}}, legend columns=2]
\nextgroupplot[bar width=3pt, xlabel={User}, xmin=0.5, xmax=8.5]
\addplot table[x expr=1+\coordindex, y index=1, col sep=comma] {plots/userStudyPerMinuteByUser.txt};
\addplot table[x expr=1+\coordindex, y index=2, col sep=comma] {plots/userStudyPerMinuteByUser.txt};
\nextgroupplot[bar width=3pt, xlabel={Article}, xticklabels={ST16,Fly,ST15,Elo,Sun,Hip}, xticklabel style={rotate=90}, legend entries={FactChecker, SQL}]
\addplot table[x expr=1+\coordindex, y index=1] {plots/userStudyPerMinuteByArticlePGF.txt};
\addplot table[x expr=1+\coordindex, y index=2] {plots/userStudyPerMinuteByArticlePGF.txt};
\end{groupplot}
\end{tikzpicture}

\ref{userThroughputLegend}
\caption{Number of claims verified per minute, grouped by user and by article.\label{userThroughputFig}}
\end{figure}


\begin{table}
\center
\caption{Results of user survey.}
%\begin{small}
\begin{tabular}{llllll}
\toprule[1pt]
\textbf{Criterion} & $\mathbf{SQL++}$ & $\mathbf{SQL+}$ & $\mathbf{SQL\approx FC}$ & $\mathbf{FC+}$ & $\mathbf{FC++}$ \\
\midrule[1pt]
Overall & 0 & 0 & 0 & 3 & 5 \\
\midrule
Learning & 0 & 0 & 0 & 2 & 6 \\
\midrule
Verification & 0 & 0 & 0 & 1 & 7 \\
\midrule
Correction & 0 & 0 & 1 & 3 & 4 \\
\bottomrule[1pt]
\end{tabular}
%\end{small}
\end{table}


\begin{table}
\caption{Comparison of fact-checking methods.}
\begin{tabular}{llll}
\toprule[1pt]
\textbf{Tool} & \textbf{Recall} & \textbf{Precision} & \textbf{F1 Score} \\
\midrule[1pt]
FactChecker + User & 100\% & 91\% & 95\% \\
\midrule
FactChecker Automatic & 67\% & 67\% & 67\% \\
\midrule
SQL + User & 30\% & 57\% & 39\% \\
\bottomrule[1pt]
\end{tabular}
\end{table}


\begin{figure}
\subfigure[test]{
\begin{tikzpicture}
\begin{axis}[ybar=0pt, bar width=2pt, width=6.5cm, height=3.5cm, xlabel=Articles, ylabel={\# Claims}, ylabel near ticks, xlabel near ticks, ymajorgrids, legend entries={Correct, Incorrect}, legend pos=outer north east, xtick=\empty, legend style={font=\small}]
\addplot table[x expr=\coordindex, y index=1] {plots/annotationTypeNrAllArticle_CorrectnessPGF.txt};
\addplot table[x expr=\coordindex, y index=2] {plots/annotationTypeNrAllArticle_CorrectnessPGF.txt};
\end{axis}
\end{tikzpicture}
}
\subfigure[a]{
\begin{tikzpicture}
\pie[radius=0.75, text=legend]{18/Zero, 70/One, 12/Two}
\node at (0,-1.5) {};
\end{tikzpicture}
}
\subfigure[a]{
\begin{tikzpicture}
\begin{axis}[width=4.5cm, height=3.5cm, xlabel=Top-N, ylabel={Coverage (\%)}, ylabel near ticks, legend entries={Function, Column, Predicates}, legend pos=south east, ymajorgrids, legend style={font=\small}]
\addplot table[x index=0, y index=1, col sep=comma] {plots/documentTopNCovergeRatio.txt};
\addplot table[x index=0, y index=2, col sep=comma] {plots/documentTopNCovergeRatio.txt};
\addplot table[x index=0, y index=3, col sep=comma] {plots/documentTopNCovergeRatio.txt};
\end{axis}
\end{tikzpicture}
}
\caption{a}
\end{figure}


\begin{figure}
\begin{tikzpicture}
\begin{axis}[ybar=0, bar width=5pt, width=5cm, height=3.5cm, ylabel=Coverage, xticklabels={Top-1, Top5, Top-10}, legend entries={Claim Sentence, +Previous Sentence, +Paragraph Start, +Synonyms, +Headlines}, legend style={font=\small}, legend pos=outer north east, xtick=data, ymajorgrids, enlarge x limits=0.2, ylabel near ticks]
\addplot table[x expr=\coordindex, y index=1] {plots/accuracyPerLucenePGF.txt};
\addplot table[x expr=\coordindex, y index=2] {plots/accuracyPerLucenePGF.txt};
\addplot table[x expr=\coordindex, y index=3] {plots/accuracyPerLucenePGF.txt};
\addplot table[x expr=\coordindex, y index=4] {plots/accuracyPerLucenePGF.txt};
\addplot table[x expr=\coordindex, y index=5] {plots/accuracyPerLucenePGF.txt};
\end{axis}
\end{tikzpicture}
\caption{a}
\end{figure}


\begin{figure}
\center
\begin{tikzpicture}[mark size=1.5pt]
\begin{groupplot}[width=4.5cm, height=3.5cm, %
group style={group size = 2 by 1, x descriptions at=edge bottom, ylabels at=edge left, horizontal sep=0.5cm},  xlabel={Time (s)}, ylabel={Coverage}, xlabel near ticks, ylabel near ticks, ymajorgrids, xmajorgrids, yminorgrids, legend columns=2, legend entries={Top-1, Top-10}, legend to name=tradeoffLegend]
\nextgroupplot
\addplot table[x index=0, y index=2, col sep=comma] {plots/timeAccuracy_AggColumn.txt};
\addplot table[x index=0, y index=3, col sep=comma] {plots/timeAccuracy_AggColumn.txt};
\nextgroupplot
\addplot table[x index=0, y index=2, col sep=comma] {plots/timeAccuracy_MaxIterationEM.txt};
\addplot table[x index=0, y index=3, col sep=comma] {plots/timeAccuracy_MaxIterationEM.txt};
\end{groupplot}
\end{tikzpicture}

\ref{tradeoffLegend}
\caption{a}
\end{figure}


\begin{figure}
\subfigure[Breakdown for small data sets.]{
\begin{tikzpicture}[font=\small]
\pie[radius=1, text = legend]{5/Idx, 24/IR, 60/EM, 10/Query}
\end{tikzpicture}}
\subfigure[Breakdown for large data sets.]{
\begin{tikzpicture}[font=\small]
\pie[radius=1, text=legend]{20/Idx, 6/IR, 7/EM, 67/Query}
\end{tikzpicture}}

\caption{Breakdown of processing time.}
\end{figure}

\begin{figure}
\begin{tikzpicture}[font=\small]
\pie[radius=1.25, text = legend]{44.5/Top-1, 38.1/Top-5, 4.6/Top-10, 12.8/Custom}
\end{tikzpicture}
\caption{a}
\end{figure}

\begin{figure}
\begin{tikzpicture}[mark size=1pt]
\begin{groupplot}[width=4.5cm, height=3.5cm, %
group style={group size = 2 by 2, x descriptions at=edge bottom, y descriptions at=edge left, horizontal sep=0.1cm}, ymin=0, xlabel={Top-N Queries}, ylabel={Coverage (\%)}, ylabel near ticks, ymajorgrids, legend to name=wtCoverageLegend, legend columns=3, legend entries={Total, Correct Claims, Incorrect Claims}, ymin=0, ymax=100]
\nextgroupplot[title=Queries]
\addplot table[x index=0, y index=1, col sep=comma] {plots/topNQueriesRatio_Correctness.txt};
\addplot table[x index=0, y index=2, col sep=comma] {plots/topNQueriesRatio_Correctness.txt};
\addplot table[x index=0, y index=3, col sep=comma] {plots/topNQueriesRatio_Correctness.txt};
\nextgroupplot[title=Functions]
\addplot table[x index=0, y index=1, col sep=comma] {plots/topNAggFunctionRatio_Correctness.txt};
\addplot table[x index=0, y index=2, col sep=comma] {plots/topNAggFunctionRatio_Correctness.txt};
\addplot table[x index=0, y index=3, col sep=comma] {plots/topNAggFunctionRatio_Correctness.txt};
\nextgroupplot[title=Aggregated]
\addplot table[x index=0, y index=1, col sep=comma] {plots/topNAggColumnRatio_Correctness.txt};
\addplot table[x index=0, y index=2, col sep=comma] {plots/topNAggColumnRatio_Correctness.txt};
\addplot table[x index=0, y index=3, col sep=comma] {plots/topNAggColumnRatio_Correctness.txt};
\nextgroupplot[title=Predicates]
\addplot table[x index=0, y index=1, col sep=comma] {plots/topNRestrictColumnRatio_Correctness.txt};
\addplot table[x index=0, y index=2, col sep=comma] {plots/topNRestrictColumnRatio_Correctness.txt};
\addplot table[x index=0, y index=3, col sep=comma] {plots/topNRestrictColumnRatio_Correctness.txt};
\end{groupplot}
\end{tikzpicture}

\ref{wtCoverageLegend}
\caption{a}
\end{figure}


\begin{table}
\caption{Total run time for all test cases.\label{totalTimeTable}}
\begin{tabular}{lll}
\toprule[1pt]
\textbf{Version} & \textbf{Run Time (s)} & \textbf{Speedup}\\
\midrule[1pt]
Naive & 5100 & -\\
\midrule
+ Query Merging & 82 & $\times62$ \\
\midrule
+ Caching & 57 & $\times1.4$ \\
\midrule
+ Incremental Evaluation & 54 & $\times1.05$ \\
\bottomrule[1pt]
\end{tabular}
\end{table}
\end{comment}

\begin{comment}
\begin{figure*}
\begin{tikzpicture}
\begin{axis}[ybar=0pt, bar width=2pt, width=14cm, height=4cm, xlabel=Articles, ylabel={Run Time (s)}, ylabel near ticks, xlabel near ticks, ymajorgrids, legend entries={Naive, Merging, Caching, Incremental}, legend pos=outer north east, xtick=\empty, legend style={font=\small}, ymode=log, enlarge x limits=0.05]
\addplot table[x expr=\coordindex, y index=1, col sep=comma] {plots/performanceAllArticles.txt};
\addplot table[x expr=\coordindex, y index=2, col sep=comma] {plots/performanceAllArticles.txt};
\addplot table[x expr=\coordindex, y index=3, col sep=comma] {plots/performanceAllArticles.txt};
\addplot table[x expr=\coordindex, y index=4, col sep=comma] {plots/performanceAllArticles.txt};
\end{axis}
\end{tikzpicture}
\end{figure*}

\begin{figure}
\begin{tikzpicture}
\begin{axis}[ybar=0pt, bar width=2pt, width=8.5cm, height=3.5cm, xlabel=Articles, ylabel={\# Queries}, ylabel near ticks, xlabel near ticks, ymajorgrids, xtick=\empty, legend style={font=\small}, ymode=log]
\addplot table[x expr=\coordindex, y index=1] {plots/nrPossibleQueriesPGF.txt};
\end{axis}
\end{tikzpicture}
\caption{a}
\end{figure}
\end{comment}
